Blended smoothing splines on Riemannian manifolds

We present a method to compute a fitting curve B to a set of data points d0,...,dm lying on a manifold M. That curve is obtained by blending together Euclidean B\'ezier curves obtained on different tangent spaces. The method guarantees several properties among which B is C1 and is the natural cubic smoothing spline when M is the Euclidean space. We show examples on the sphere S2 as a proof of concept.

==> pics/sphere_fitting_dist.tex <==

\begin{axis}[
	axis x line = bottom,
	axis y line = left,
	enlarge x limits=0.05,
	enlarge y limits=0.05, 
	xlabel={$t$},
	%ylabel={$\mathrm{E}[\| \ddot \bspline(t) \|]$},
	%x label style={font=\footnotesize},
	%xlabel style={at=(current axis.right of origin), anchor=south west},
	%ytick={-3.1416,  -1.5708, 0, 1.5708, 3.1416}, yticklabels={$-\pi$, $-\frac{\pi}2$, 0, $\frac\pi2$, $\pi$},
	%y label style={at={(axis description cs:0.12,.5)},anchor=south,},% font=\footnotesize},
	%ticklabel style = {font=\footnotesize},
	%scale=.9,
	ymax = 0.05,
	ymin = -0.05,
	height=4cm,
	width=7cm
	]
	
	% Curve
	\addplot [bezier]
		table [x=x,y=y]
		{pics/figure2/data-sphereFit_dist.dat}
		;

		
\end{axis}

